BulletTrain: Accelerating Robust Neural Network Training via Boundary Example Mining

Neural network robustness has become a central topic in machine learning in recent years. Most training algorithms that improve the model's robustness to adversarial and common corruptions also introduce a large computational overhead, requiring as many as ten times the number of forward and backward passes in order to converge. To combat this inefficiency, we propose BulletTrain $-$ a boundary example mining technique to drastically reduce the computational cost of robust training. Our key observation is that only a small fraction of examples are beneficial for improving robustness. BulletTrain dynamically predicts these important examples and optimizes robust training algorithms to focus on the important examples. We apply our technique to several existing robust training algorithms and achieve a 2.1$\times$ speed-up for TRADES and MART on CIFAR-10 and a 1.7$\times$ speed-up for AugMix on CIFAR-10-C and CIFAR-100-C without any reduction in clean and robust accuracy.

==> backup.tex <==
\begin{figure}[!t]
        \centering
        \begin{subfigure}{0.48\linewidth}
            \centering
            \includegraphics[scale=0.4]{fig/eps_robust.png}
            \caption{Robust accuracy.}
            \label{fig:eps_robust}
        \end{subfigure}
        \hspace{0.2cm}
        \begin{subfigure}{0.48\linewidth}
            \centering
            \includegraphics[scale=0.4]{fig/eps_natural.png}
            \caption{Natural accuracy.}
            \label{fig:eps_natural}
        \end{subfigure}
        \caption{Comparisons of accuracy at different $\epsilon$.}
    \label{fig:eps}
\end{figure}

\subsection{Algorithm}
\textbf{Separate the clean samples.}
Among the three sets of examples, the outlier examples can be separated easily as the outlier examples are misclassifided by the current DNN model.
Therefore, we can use the sign of prediction defined as follows:
\begin{equation}
\textnormal{Sign of prediction} = \begin{cases}
               +1,& \text{if } \argmax_{k=1,...K} h_\theta^k(\mathbf{x}) = y\\ 
               -1,& \text{otherwise}\\
            \end{cases}
\end{equation}

In addition, we need to distinguish between the boundary and robust examples, where the boundary examples are closer to the decision boundary than the robust ones.
As suggested in prior arts on importance sampling~\citep{active_bias}, the prediction variance ($\textnormal{Var}[\Softmax(h_\theta(\mathbf{x}))]$) can be used to measure the uncertainty of each sample for a classification problem, where $\textnormal{Var}[\cdot]$ and $\Softmax(\cdot)$ stand for variance and normalized exponential function respectively.
The samples with low uncertainty are typically far from the decision boundary than the samples with high uncertainly.
In other words, the prediction variance also indicates the distance between the sample and the decision boundary, which can be leveraged to separate between $\mathbf{x}_B$ and $\mathbf{x}_R$.
We combine the sign of prediction and the prediction variance by multiplying the sign and variance as the final metric (signed prediction variance $\text{SVar}[\cdot]$).
As shown in Figure~\ref{fig:pred_var}, the signed prediction variances of $\mathbf{x}_R$, $\mathbf{x}_B$, and $\mathbf{x}_O$ from different mini-batches are mostly rank correlated ($\text{SVar}[\mathbf{x}_O] < \text{SVar}[\mathbf{x}_B] < \text{SVar}[\mathbf{x}_R]$), which suggests that the proposed metric can be leveraged to differentiate between different types of samples.
We also consider other possible metrics such as natural cross-entropy loss $\CE(h_\theta(\mathbf{x}))$ and the upper bound of gradient norm derived in~\citep{graident_norm}.
Since these metrics perform similar to the prediction variance, we stick to the signed prediction variance metric.

As the goal of \name~is to reduce the computational cost, it requires an efficient way of predicting the class of samples based on the signed prediction variance.
To make the prediction with minimal compute, we proposed to predict the class of samples by estimating the fraction of $\mathbf{x}_R$, $\mathbf{x}_B$, and $\mathbf{x}_O$.
The fraction of $\mathbf{x}_O$ ($F_{O}$) can be obtained accurately by calculating the natural error rate:
\begin{equation}
    F_O = 1-\frac{\sum_i^m \mathds{1}(\argmax_k h_\theta^k(\mathbf{x}_i) = y_i)}{m}
\end{equation}
where $\mathds{1}(\cdot)$ is the indicator function.
The fraction of $\mathbf{x}_R$ or $\mathbf{x}_B$ can not be computed directly without generating the corrupted samples.
Therefore, we estimate the fraction of $\mathbf{x}_R$ ($F_R$) of current mini-batch using the momentum-based moving average of the robust accuracy of previous mini-batches, as the robust accuracy of the model should be reasonably consistent across different randomized mini-batches:
\begin{equation}
    F_R \leftarrow p \cdot F_R + (1-p) \cdot \frac{\sum_i^m \mathds{1}(\argmax_k h_\theta^k(\mathbf{x}'_i) = y_i)}{m}
\end{equation}
where $\mathbf{x}'$ are the corrupted samples of the previous mini-batch, $p$ is the momentum, and $F_R$ is initialized to be zero.
As illustrated in Figure~\ref{fig:scheme_hist}, $\mathbf{x}_B$ and $\mathbf{x}_R$ are not completely separable using the signed prediction variance.
To make a conservative prediction for the robust examples, we scale the $F_R$ with a scaling factor $\gamma$, where $\gamma \in [0, 1]$.

\begin{figure}[t]
\centering
\includegraphics[scale=0.9]{fig/histogram.pdf}
\caption{The distribution of signed variance of prediction of a mini-batch --- \small{The number of steps $N_R$, $N_O$, and $X_B$ for $\mathbf{x}_R$, $\mathbf{x}_O$, and $\mathbf{x}_B$ are determined by estimating the fraction of each class of samples in the mini-batch. }}
\label{fig:scheme_hist}
\end{figure}

Given the $F_O$ and $F_R$, we can first compute the signed prediction variances for all clean examples as {$\text{SVar}_{1...m} = \{{\text{SVar}}[h_\theta(\mathbf{x}_1)], ..., \text{SVar}[h_\theta(\mathbf{x}_m)]\}$}.
Then, the non-parametric classification function ($f$) can be formulated as:
\begin{equation}
f(\mathbf{x}_i, F_O, F_R) = \mathbf{x}_i \in\begin{cases}
                \mathbf{x}_O, & \text{if}~{\text{SVar}}[h_\theta(\mathbf{x}_i)] < \text{Percentile}(\text{SVar}_{1...m}, P_O)\\ 
                \mathbf{x}_R, & \text{if}~{\text{SVar}}[h_\theta(\mathbf{x}_i)] > \text{Percentile}(\text{SVar}_{1...m}, 1-P_R)\\
                \mathbf{x}_B, & \text{otherwise}\\
            \end{cases}
\end{equation}
where the Percentile$(\mathbf{X}, q)$ returns the $q^{th}$ percentile of $\mathbf{X}$.
The computational cost of $f$ comes mostly from obtaining the logits of clean example $h_\theta(\mathbf{x})$, which is already computed in robust DNN training.
Therefore, the overhead of separating between the robust, boundary, and outlier samples is negligible.

\textbf{Compute allocation scheme.}
After categorizing the clean examples into three classes, it is relatively straightforward to allocate computational cost for each class of samples.
We introduce the number of iterations (i.e., steps) for boundary ($N_B$), robust ($N_R$), and outlier ($N_O$) examples as three hyperparameters.
$N_B$ is the same as the number of steps $N$ in the original robust DNN training algorithm. 
Based on the importance of $\mathbf{x}_O$,  $\mathbf{x}_R$,  $\mathbf{x}_B$, we set $N_O \leq N_R \leq N_B$ as illustrated in Figure~\ref{fig:scheme_hist}.
Here, we present the full algorithm of \name~in Algorithm~\ref{list:scheme}.

\begin{algorithm}
\footnotesize{
\SetNoFillComment
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
    \Input{batch size $m$, DNN classifier parameterized by $\theta$, a $N$-step process for generating corrupted samples $G$,  classification function $f$, momentum of moving average $p$}
    \Output{robust DNN classifier $h_\theta$}
     $F_O \leftarrow 0; F_R \leftarrow 0$\\
     \While{$\theta$ \textnormal{not converged}}{
     Read mini-batch $\{\mathbf{x}_1, ..., \mathbf{x}_m; y_1,...,y_m\}$ from training set\\
     $\{\mathbf{z}_1, ..., \mathbf{z}_m\} \leftarrow \{h_\theta(\mathbf{x}_1),...,h_\theta(\mathbf{x}_m)\}$\\
     $F_O \leftarrow  1-\sum_i^m \mathds{1}(\argmax_k (z_i)^k = y_i)/m$\\
    $\mathbf{x}_R, \mathbf{x}_B, \mathbf{x}_O \leftarrow f(\{\mathbf{x}_1,...,\mathbf{x}_m\}, F_O, F_R)$\\
    \For{$j = 1,..., N_O$}{
        $\mathbf{x}'_R \mathbin\Vert \mathbf{x}'_B \mathbin\Vert \mathbf{x}'_O\leftarrow G(\mathbf{x}_R \mathbin\Vert \mathbf{x}_B \mathbin\Vert \mathbf{x}_O)$
    }
    \For{$k = 1,..., N_R-N_O$}{
        $\mathbf{x}'_R \mathbin\Vert \mathbf{x}'_B \leftarrow G(\mathbf{x}'_R \mathbin\Vert \mathbf{x}'_B)$
    }
    \For{$l = 1,..., N_B-N_R$}{
        $\mathbf{x}'_B \leftarrow G(\mathbf{x}'_B)$
    }
     $\{\mathbf{x}'_1,...,\mathbf{x}'_m\} \leftarrow \mathbf{x}'_R \mathbin\Vert \mathbf{x}'_N \mathbin\Vert \mathbf{x}'_O$; $\{\mathbf{z}'_1, ..., \mathbf{z}'_m\} \leftarrow \{h_\theta(\mathbf{x}'_1),...,h_\theta(\mathbf{x}'_m)\}$\\
     $F_R \leftarrow p \cdot F_R + (1-p) \cdot \sum_i^m \mathds{1}(\argmax_k (\mathbf{z}'_i)^k = y_i)/m$\\
     $\theta \leftarrow \theta - \nabla_{\theta}(\mathcal{L}(\{\mathbf{z}_1, ..., \mathbf{z}_m\}, \{\mathbf{z}'_1, ..., \mathbf{z}'_m\}))$
     }
 \caption{\name.}
 \label{list:scheme}
 }
\end{algorithm}

\name~first separates a mini-batch of samples into robust, boundary, and outlier samples dynamically based on the signed prediction variance.
The separation is relatively accurate as the signed prediction variance can capture the distance between samples and the decision boundary of the current model.
Then, the outlier, robust, boundary examples take $N_O$, $N_R$, and $N_B$ steps to generate the corresponding corrupted samples, respectively.
As only a small fraction of samples (i.e., boundary examples) requires executing the same number of iterations as the baseline, the computational cost is reduced significantly.
Lastly, the surrogate loss is computed with respect to the natural and corrupted samples.
If both $N_O$ and $N_R$ are equal to zero, the corrupted sample remains the same as the original sample, and thus eliminating the extra cost for computing the surrogate loss and backpropagation for the corrupted sample. 

For adversarial training, the main saving of applying \name~stems from reducing the number of steps for robust and boundary examples since the original adversarial training algorithms typically adopt a large numbers of steps.
On the contrary, the reduction in compute for robust training against natural corruptions mostly comes from not computing the surrogate loss and backpropagation for corrupted samples.
For example, as shown in Equation~\ref{eq:augmix}, the computational cost of AugMix can be lowered by half if we only generate the corrupted samples for half of clean samples in the mini-batch.

After obtaining the estimated fraction of the outlier and robust examples, we can assign the number of steps for each sample following our intuition discussed in Section~\ref{sec:intuition}.
Figure~\ref{fig:scheme_hist} shows that $\mathbf{x}_B$ and $\mathbf{x}_R$ are not completely separable using the signed prediction variance.
In other words, the type of samples near the boundary between $\mathbf{x}_B$ and $\mathbf{x}_R$ is fairly unpredictable.
Therefore, we propose to focus on samples in the region around the boundary between $\mathbf{x}_B$ and $\mathbf{x}_R$.

We introduce bandwidth $B$ as a hyperparameter and spend the largest number of steps ($N_H$) on the samples whose signed prediction variance is between $F_{-}$ and $F_{+}$ percentiles of all samples in the same mini-batch, where $F_{-}=1-F_R-B/2$, $F_{+}=1-F_R+B/2$, and $B \in [0, 1]$.
For the rest of the samples, we allocate the second largest number of steps ($N_M$) for the samples whose signed predicting variance is positive (i.e., larger than $F_{O}$ percentiles of all samples). 
Lastly, the outlier examples receive the lowest number of steps ($N_L$).

\iffalse
In addition to boosting the adversarial robustness, there is also a line of research on reducing the cost of adversarial training~\citep{free, yopo, fast}.
YOPO~\citep{yopo} proposes to skip the redundant computation in backpropagation when generating adversarial examples, which is orthogonal to our proposal.
Both Free~\citep{free} and Fast~\citep{fast} suggest using a variant of single-step FGSM adversarial training to replace the $N$-step PGD training, which can reduce the cost of adversarial training significantly.
However, the single-step FGSM adversarial training approaches might suffer from a phenomena called "catastrophic overfitting"~\citep{fast, understand_fast}, where the adversarial accuracy can drop to zero during the training process. 
\cite{understand_fast, smooth_backprop} further improves the robustness of single-step FGSM by maximizing the gradient alignment in the perturbations or smoothing the initialization randomly .
Compared to prior works on efficient adversarial training, \name~leverages the input characteristic (i.e., margin) and only reduces the number of steps for non-important samples at run time.
As a result, \name~can lower the computational cost of adversarial training without sacrificing the strong robustness obtained from PGD training and its variants.  
\fi

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
     \answerYes{} The main claims are clearly stated in the introduction.
  \item Did you describe the limitations of your work?
    \answerYes{} We discussion the limitation of this work in the conclusion and feature Work section.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{} This work should have no negative societal impacts as this paper aims to accelerate robust neural network training and make neural networks more robust to attacks.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} We will include the code, data, and instructions in the supplemental material.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} Most important details are presented in the experiment section and minor details are reflected in the supplemental material.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{} As the variance of accuracy is small, we do not report error bars.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} We report the type and number of GPUs in the experiment section.

\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{} We fail to find the license for CIFAR-10 and CIFAR-100.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} Our code will be included in the supplemental material.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}{} We use public datasets such as CIFAR-10 and CIFAR-100.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{} We believe that the datasets do not contain any personally identifiable information.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
